Locomotion Generation for a Rat Robot based on Environmental Changes via Reinforcement Learning

This research focuses on developing reinforcement learning approaches for the locomotion generation of small-size quadruped robots. The rat robot NeRmo is employed as the experimental platform. Due to the constrained volume, small-size quadruped robots typically possess fewer and weaker sensors, resulting in difficulty in accurately perceiving and responding to environmental changes. In this context, insufficient and imprecise feedback data from sensors makes it difficult to generate adaptive locomotion based on reinforcement learning. To overcome these challenges, this paper proposes a novel reinforcement learning approach that focuses on extracting effective perceptual information to enhance the environmental adaptability of small-size quadruped robots. According to the frequency of a robot's gait stride, key information of sensor data is analyzed utilizing sinusoidal functions derived from Fourier transform results. Additionally, a multifunctional reward mechanism is proposed to generate adaptive locomotion in different tasks. Extensive simulations are conducted to assess the effectiveness of the proposed reinforcement learning approach in generating rat robot locomotion in various environments. The experiment results illustrate the capability of the proposed approach to maintain stable locomotion of a rat robot across different terrains, including ramps, stairs, and spiral stairs.

==> relatedwork.tex <==
\section{Related Work}
% In nature, small quadrupedal animals exhibit strong adaptability to different environments due to their small size and high agility. Inspired by this, researchers have developed small-size quadruped robots for exploration tasks in narrow spaces through design bionics. However, with physical hardware constraints, the flexibility of small-size quadruped robots always lags significantly behind that of their biological prototype.

% To enhance the flexibility of robots and adapt to different environmental changes, researchers have introduced additional DOFs for small-size quadruped robots, enabling them to perform a wider range of locomotion. Analyzing the behaviors of real rats, Qing et. al. developed a rigid spine consisting of multiple joints for their rat robots \cite{shi2018modified, shi2020implementing}. With the imitation of various rat locomotion, their robot is capable of coupling spinal motion with quadrupedal locomotion, thus enhancing its mobility, agility, and obstacle-crossing ability \cite{wang2019design, shi2022development}. In narrow spaces, their robot performs excellently by executing a variety of bioinspired locomotion. Bing et. al. designed a soft-actuated spine controlled by a single DOF, inspired by the skeletal structure of natural rat \cite{lucas2019development, bing2023lateral}. They modeled the dynamic coordination mechanism between continuous spinal flexion and quadrupedal locomotion \cite{huang2022enhanced}. By dynamically adjusting the curvature of the spine based on limb locomotion, they improved the robot's performance in various aspects, including minimum turning radius, movement speed, and dynamic balance \cite{huang2022enhanced, bing2023lateral, huang2024optimizing}. They also developed a CPG model driven by spinal motion to support smooth gait transitions for the robot under changing environmental demands \cite{huang2023smooth}. While the above methods effectively enhance the robot's adaptability to environments, they require specific action sequences tailored to particular environments. For uncertain environments, their control model's generalization ability is limited. This is because the complexity of the environment results in significant challenges to the design of robot control models. To enhance the robot's adaptability to various environments, RLs that can extract adaptive motions for different environments from a large amount of simulation data are a potentially feasible solution.


% Reinforcement learning, as a trial-and-error-based learning approach, has been successfully applied to learning the gaits of robots. Through interaction with the environment, robots can autonomously learn near-optimal policies of robot locomotion to adapt to complex and changing environmental conditions. Researchers at the Robotic Systems Lab at ETH Zurich have used RL to learn flexible gaits for robots without excessive manual intervention \cite{hwangbo2019learning}. To address the issue of reinforcement learning being strongly correlated with a single environment, they employed hierarchical reinforcement learning to guide the robot in generating optimal locomotion in response to continuous environmental changes during real tasks \cite{lee2020learning, miki2022learning, jenelten2024dtc}. Moreover, to enhance the robot's learning capability, Shi et.al. designed an evolutionary trajectory generator for reinforcement learning to simplify the robot's action space when generating robot gaits \cite{shi2022reinforcement}. This method increases the possibilities of discovering optimal adaptive locomotion. However, the aforementioned approaches are designed for full-size quadruped robots and are difficult to apply to small-size robots. This is because small-size robots, constrained by their size, exhibit underactuated and underperceived characteristics. In this case, small-size quadruped robots hard to meet the diverse sensory information and precise motion execution requirements demanded by existing RL approaches.


% To address the above issues, this paper aims to develop an RL approach towards robots with weak perception. With this approach, small-size quadruped robots can learn adaptive locomotion to adapt to various environmental changes.

Drawing from the adaptability of small quadrupeds in nature, small-sized quadruped robots have been developed for exploration in confined spaces, albeit with limitations in flexibility compared to their biological counterparts. To improve this, researchers have enhanced robot flexibility by adding Degrees Of Freedom (DOFs), as seen in Qing et al.'s rat robot with a multi-joint spine \cite{shi2018modified, shi2020implementing}, and Bing et al.'s design featuring a soft-actuated spine \cite{lucas2019development, bing2023lateral}. These innovations boost mobility and adaptability but are often tailored to specific environments, limiting their applicability in unpredictable settings due to control model complexities.

Reinforcement Learning (RL) has emerged as a promising solution, enabling robots to learn adaptive locomotion through trial-and-error interactions with the environment. Notably, ETH Zurich's Robotic Systems Lab has applied RL for flexible gait learning \cite{hwangbo2019learning}, while hierarchical RL has been utilized to accommodate continuous environmental changes \cite{lee2020learning, miki2022learning, jenelten2024dtc}. Despite successes, the direct application of these RL strategies to small-sized robots remains challenging due to their underactuated and underperceived nature.

This paper proposes an RL approach tailored for robots with limited sensory capabilities, allowing small-sized quadruped robots to adapt to diverse environmental changes through learned adaptive locomotion.

